Bandits with Knapsacks beyond the Worst-Case

Bandits with Knapsacks (BwK) is a general model for multi-armed bandits under supply/budget constraints. While worst-case regret bounds for BwK are well-understood, we present three results that go beyond the worst-case perspective. First, we provide upper and lower bounds which amount to a full characterization for logarithmic, instance-dependent regret rates. Second, we consider "simple regret" in BwK, which tracks algorithm's performance in a given round, and prove that it is small in all but a few rounds. Third, we provide a general "reduction" from BwK to bandits which takes advantage of some known helpful structure, and apply this reduction to combinatorial semi-bandits, linear contextual bandits, and multinomial-logit bandits. Our results build on the BwK algorithm from \citet{AgrawalDevanur-ec14}, providing new analyses thereof.

==> LB-log.tex <==
\section{Logarithmic lower bound}
\label{sec:LB-log} 

\ascomment{just copied from the "old" LB section.}

Our first lower bound concerns the dependence on $\Dmin$, and holds for any given value thereof.

\begin{theorem}[dependence on $\Dmin$]\label{thm:mainLB}
Posit an arbitrary time horizon $T$, budget $B = \nicefrac{T}{2}$, and $d=2$ resources (including time). For any
    $\eps\in(\nicefrac{1}{\sqrt{T}},\nicefrac{1}{4})$,
there exist two $3\times 2$ problem instances $\mI$, $\mI'$ with $\Dmin=\eps/2$ such that any algorithm incurs regret
$\OPTFD-\E[\REW] \geq \Omega\rbr{\Dmin^{-2}}$
on either $\mI$ or $\mI'$.
In fact, both problem instances have deterministic resource consumption.
\end{theorem}

The problem instances for Theorem~\ref{thm:mainLB} are constructed as follows. For arm $A_1$, resource consumption is deterministically  $\nicefrac{1}{2}$, and reward is drawn from
    $\term{Bernoulli}(\nicefrac{1}{4})$.
 For arm $A_2$, the consumption is deterministically $1$, and the reward is drawn from
    $\term{Bernoulli}(\nicefrac{1}{2} \pm \nicefrac{\eps}{2})$.
\footnote{That is, the reward for arm $A_2$ is
    $\term{Bernoulli}(\nicefrac{1}{2} + \nicefrac{\eps}{2})$
for one instance, and
    $\term{Bernoulli}(\nicefrac{1}{2} - \nicefrac{\eps}{2})$
for another.}
That $\Dmin$ is as claimed follows immediately from the construction.
Because of the small difference between the two instances, any algorithm will choose a ``wrong" arm at least $\Omega(\eps^{-2})$ times on one of the instances, which in turn implies $\Omega(\eps^{-2})$ regret. The full proof is in Section~\ref{sec:LB-gap}.


\ascomment{the rest is the proof}

Let $\vX^*_\mJ$ be the optimal distribution over arms for the linear relaxation \eqref{lp:primalAbstract} of a given problem instance $\mJ$.
$\vX^*_\mI$ chooses arm $A_1$ with probability $1$, giving an instantaneous expected reward of $\nicefrac{1}{4}$ on instance $\mI$. $\vX^*_{\mI'}$ randomizes uniformly between arm $A_2$ and the null arm. Its instantaneous expected reward on instance $\mI'$ is $\nicefrac{1}{4} + \nicefrac{\eps}{2}$. In both problem instances, $\Dmin = \nicefrac{\eps}{2}$.

Consider an arbitrary algorithm \ALG. Apply Lemma~\ref{lem:bestArm} with \LBrewards as rewards, and
    \[ H := \{\text{distribitions } \vX:
        \| \vX- \vX^*_\mI \|_1  \geq \tfrac{3}{4} \}.\]

\kaedit{Let $\vec{Y}_t$ denote the distribution chosen by the algorithm at time $t$. If $\vec{Y}_t \in H$, by definition this implies that $\| \vY_t- \vX^*_\mI \|_1  \geq \tfrac{3}{4}$. If $\vec{Y}_t \notin H$, by definition this implies that $\| \vY_t- \vX^*_\mI \|_1  < \tfrac{3}{4}$. This can be rewritten as $\| \vY_t- \vX^*_{\mI'} + \vX^*_{\mI'} - \vX^*_\mI \|_1  < \tfrac{3}{4}$. Using triangle inequality and the definitions of the distributions $\vX^*_\mI$ and $\vX^*_{\mI'}$, this implies that $\tfrac{5}{4} \leq \| \vY_t- \vX^*_{\mI'} \| \leq \tfrac{11}{4}$.}

\kaedit{We also use the following algebra in the proof. First, note that for any two distributions $\vec{X}, \vec{Y} \in \Delta_K$, we have $\| \vec{X} - \vec{Y} \|_1 = 2 \cdot \sum_{j \in [K]: X_j \geq Y_j} X_j - Y_j$. Next, if $\| \vec{X} - \vec{Y} \|_1 \geq \alpha$, this implies that there exists a $j \in [K]$ such that $X_j - Y_j \geq \frac{\alpha}{2K}$. }

We now use the above observation to complete the proof. \asedit{We pick $\eps$ such that $T = \frac{c}{\eps^2}$. We apply the lemma to each round $t\in [T]$, and let
    $\mJ_t \in \{ \mI,\, \mI' \}$
be the corresponding problem instance guaranteed by the lemma. If $\mI$ appears in this sequence at least $T/2$ time/y5s we have the following.}

The expected regret incurred by $\ALG$ is at least
\begin{align*}
&\sum_{t \in [T]:\; \mJ_t = \mI} \E\sbr{ \mathbb{I}[\vec{Y}_t \in H]} \cdot \langle \vX^*_\mI - \vec{Y}_t, \vec{r} \rangle
\\
& \qquad \sum_{t \in [T]:\; \mJ_t = \mI} 2 \cdot \E\sbr{ \mathbb{I}[\vec{Y}_t \in H]} \cdot \left( \sum_{j \in [K]: X^*_{\mI}(j) \geq Y(j)}  X^*_{\mI}(j) - Y(j) \right)
&\qquad\geq \sum_{t \in [T]:\; \mJ_t = \mI} \E\sbr{ \mathbb{I}[\vec{Y}_t \in H]} \cdot ( \vX^*_\mI(j) - \vec{Y}_t(j) ) \cdot \left( \min_{j \in [3]} r_j \right)
    & \EqComment{by triangle inequality} \\
&\qquad\geq \frac{c}{2 \eps^2} \cdot \nicefrac{1}{4} \cdot \nicefrac{3}{4} \cdot \rbr{\nicefrac{1}{4} - \eps}
    & \EqComment{by defn. of $H$ and the construction}\\
		&\qquad\geq \Omega\rbr{\eps^{-2}} = \Omega\rbr{\Dmin^{-2}}.
	\end{align*}

Likewise, if $\mI'$ appears in this sequence at least $T/2$ times, then the expected regret incurred by $\ALG$ is at least,

\begin{align*}
&\sum_{t \in [T]:\; \mJ_t = \mI'} \E\sbr{ \mathbb{I}[\vec{Y}_t \notin H]} \cdot \langle \vX^*_{\mI'} - \vec{Y}_t, \vec{r} \rangle
\\
&\qquad\geq \sum_{t \in [T]:\; \mJ_t = \mI'} \E\sbr{ \mathbb{I}[\vec{Y}_t \notin H]} \cdot \| \vX^*_{\mI'} - \vec{Y}_t \|_1 \cdot \left( \min_{j \in [3]} r_j \right)
    & \EqComment{by triangle inequality} \\
&\qquad\geq \frac{c}{2 \eps^2} \cdot \nicefrac{1}{4} \cdot \nicefrac{5}{4} \cdot \rbr{\nicefrac{1}{4} - \eps}
    & \EqComment{by defn. of $H$ and the construction}\\
		&\qquad\geq \Omega\rbr{\eps^{-2}} = \Omega\rbr{\Dmin^{-2}}.
	\end{align*}


%Sketch of the proof
%		\begin{enumerate}
%			\item Show that the rescaled LP is a lower-bound on OPTFD (We can cite our focs paper, where this is proved)
%			\item Show that pertubation does not change the LP optimal basis (we can use sensitivity theor64bcdf8bem since the constraints are linearly independent)
%			\item Show that the tight constraints do not change (Need to add this to the assumption).
%			\item Then the proof below goes through!
%		\end{enumerate}	


==> algorithm.tex <==
\section{Logarithmic regret bounds [OBSOLETE!]}
\label{sec:algorithm}

We analyze a version of \UCBBwK which ``prunes out" the null arm, call it \FinalAlgName.%
\footnote{This modification can only improve regret, so it retains the near-optimal worst-case performance of \UCBBwK.}
We prove that this algorithm enjoys logarithmic instance-dependent regret bounds under two assumptions: $d=2$ (only one resource other than time) and best-arm-optimality (Definition~\ref{def:best-arm-optimal}). These assumptions are essentially necessary to improve over $\Omega(\sqrt{T})$ regret (see Section~\ref{sec:LB}).

\asedit{We make these two assumptions throughout this section, unless specified otherwise. The best arm is denoted $a^*$. We use $c(a)$ to denote the mean consumption of the non-time resource on arm $a$. Our results have two cases, depending on whether $c(a^*)$ is very close to $\nicefrac{B}{T}$.}

%\asmargincomment{This would probably go to the intro.}
%\asedit{We match the logarithmic regret bound \eqref{eq:logT-bandits} for bandits without budget constraints in terms of the Lagrangian gap $\Dmin$, unless $c(a^*)$ is very close to $\nicefrac{B}{T}$. In the latter case, we can only achieve $\mO(\Dmin^{-2} \log T)$ regret, which we prove is optimal.}

%\subsection{Algorithm and results}

\OMIT{To simplify presentation, we first define an algorithm that uses the null arm, and then transform it so that the null arm is ``pruned". To make this well-defined, the algorithm runs indefinitely until it is stopped. All regret bounds are proved for the ``pruned" version.}

\OMIT{ %%%%%%
Our algorithm is the $\UCBBwK$ algorithm from \cite{AgrawalDevanur-ec14}, defined in Section~\ref{sec:prelims-conf}, with additional exploration steps that are crucial for obtaining logarithmic regret. In a given round $t$, we compute the solution $\vX_t$ to the optimistic LP~\eqref{lp:UCBBwK}, and sample from this distribution. See Algorithm~\ref{alg:UCBBwK}.

	\begin{algorithm2e}[!h]
		\caption{Algorithm \AlgName}
		\label{alg:UCBBwK}
			\DontPrintSemicolon
			\SetKwInOut{Input}{input}
			\Input{parameters $B,K,d,T$.}
				 Initialize $t = 1$. \;
				\While{the algorithm is not stopped}{
				\begin{minipage}{15cm}
				\begin{enumerate}[topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex]
					\item \label{alg:LPSolving} \underline{\textbf{Solve LP.}}
Obtain optimal solution $\vX = \vX_t$ to the optimistic LP~\eqref{lp:UCBBwK}.\;
                    \item \label{alg:mainSample} \underline{\textbf{UCB-round.}}
                    Sample arm $a_t$ from distribution $\vX$. \;
					\item Advance round $t\leftarrow t+1$ \;
		\end{enumerate}
		\end{minipage}
		}
		\end{algorithm2e}
} %%%%%%

Algorithm \FinalAlgName is formally defined as follows: in each round $t$, call \AlgName as an oracle, repeat until it chooses a non-null arm $a$, and set $a_t=a$. (In one ``oracle call", \AlgName outputs an arm and inputs an outcome vector for this arm.) The algorithm stops after it makes the total of $\Nmax$ oracle calls,%
\footnote{Equivalently, then the algorithm can output the null arm in all subsequent rounds.}
where
%\begin{align}\label{eq:Nmax}
 $\Nmax = \Theta(T^2\;\log T)$
(with a sufficiently large absolute constant).
%\end{align}


%	We prove logarithmic regret bounds for Algorithm~\ref{alg:UCBBwK} when the following assumptions hold.
%	\begin{assumption}
%	\label{subsec:assmps}
%	\setlist[enumerate,1]{label={(\roman*)}}
%	\begin{enumerate}
%		\item \label{ass:optimalSingleArm} The optimal solution to $\LP$~\eqref{lp:primalAbstract} is unique and is supported on either one arm $a^* \in [K]$ or two arms of which one is the null arm.\footnote{A-priori, the algorithm doesn't know $a^*$.}
%		% \item \label{ass:budget} The total budget $B$ is a constant fraction of $T$ (\ie $B \geq \Omega(T)$).
%		\item The Lagrangian gap satisfies
%            $\Dmin \geq 2\;\DminLB$.
%		\item One of the following two hold.
%			\begin{enumerate}[label=\textbf{(A.\arabic*)},ref=Assumption (A.\arabic*)]
%				\item \label{ass:deterministicCost} The resource consumption for every resource $j \in [d]$ and every action $a \in [K]$ are deterministic across time. Thus, wlog we assume that the algorithm knows the consumption of each resource for all actions before its start.\footnote{The algorithm can play each action once in the beginning and obtain this}
%				\item \label{ass:singleResource}  We have exactly two resources: time and one other resource. We do not require this other resource to be deterministic. Wlog we assume that the expected consumption vector for this resource is not a scalar multiple of the all ones vector.
%		\end{enumerate}
%	\end{enumerate}
%	\end{assumption}





%Consider a problem instance $\mathcal{I}$ satisfying Assumption~\ref{subsec:assmps}. Consider \AlgName~described in Algorithm~\ref{alg:UCBBwK}, that knows if $\mathcal{I}$ satisfies \ref{ass:deterministicCost}. If it does, Algorithm~\ref{alg:UCBBwK} sets $\UCB$ and $\LCB$ for every resource $j \in [d]$ to be the known deterministic value in all time-steps $t \in [T]$. If not, they are as defined in \refeq{eq:confidencebounds}. Let $\REW$ denote the total reward obtained by the algorithm. Then with probability at least $1-\frac{1}{\poly(T)}$ we have,

\begin{theorem}\label{thm:logRegretUpper}
Suppose there is only one resource other than time (\ie $d=2$),
and
    $\myEta\leq \tfrac12$ in \eqref{eq:prelims-eta}.
Consider a best-arm-optimal instance $\mI$ with Lagrangian gap
            $\Dmin > 0$.
%Assume either one of the following:
%\begin{OneLiners}
%\item[(a)] there is only one resource other than time (\ie $d=2$),
%\item[(b)] the resource consumption is deterministic and known, in the sense of~\eqref{eq:known-consumption}.
%\end{OneLiners}
\begin{itemize}
\item[(i)] Algorithm \FinalAlgName achieves regret
\begin{align}\label{eq:logRegretSecondEq}
			\OPTFD - \E[\REW] \textstyle
    \leq  \mO\rbr{
        \sum_{a \neq a^*} \DGap^{-2}(a)\; \logThm}.
\end{align}

\item[(ii)]
Moreover, if
    $|c(a^*)-\nicefrac{B}{T}| >
        \mO\rbr{\nicefrac{B}{T}\cdot \sqrt{\nicefrac{K}{B}\cdot \logThm}} $ then
	\begin{align}\label{eq:logRegretMainEq}
	\OPTFD - \E[\REW] \textstyle
    \leq \mO\rbr{
        \sum_{a \neq a^*} \DGap^{-1}(a)\; \logThm\; + \OPTFD/B }.
    \end{align}
\end{itemize}
%s\asedit{assuming a sufficiently large absolute constant in $\Theta()$ in \eqref{eq:Nmax}.}
\end{theorem}

\OMIT{ %%%%%
\begin{theorem}[worst-case]\label{thm:worst-case}
Assume $\myEta\leq \tfrac12$ in \eqref{eq:prelims-eta}.
%with a sufficiently large absolute constant in $\mathcal{O}()$.
Then \FinalAlgName achieves
\begin{align}\label{eq:WSRegret}
\OPTDP - \E[\REW]	
\leq \mO\left( \sqrt{\logThm}
    \left( \OPTDP\sqrt{\nicefrac{K}{B}}  + \sqrt{K\,\OPTDP} \right)
        \right).
\end{align}
\end{theorem}

\begin{remark}\label{rem:logRegret-worstCase}
\refeq{eq:WSRegret} is the worst-case optimal regret bound \eqref{eq:regret-opt} and follows directly from the analysis in \cite{AgrawalDevanur-ec14}. \kacomment{We don't need to prove anything here.}
\end{remark}
} %%%%%

%	\begin{remark}
%		\label{rem:nullArm}
%		Given an oracle access to an algorithm $\mathcal{A}$ that plays the null arm in some time-steps, we can construct another $\mathcal{A}'$ that does not play the null-arm untwhile having the same regret bounds. At each time-step $t \in [T]$, algorithm $\mathcal{A}'$ makes an oracle call to algorithm $\mathcal{A}$. If the returned action is a null-action, $\mathcal{A}'$ does play this action and makes another call to $\mathcal{A}$. If for $T$ consecutive oracle calls, the returned action is a null-action $\mathcal{A}'$ stops the game. This ensures that the feedback obtained by algorithm $\mathcal{A}$ is the same as that of $\mathcal{A}'$ and thus, not affecting the total expected reward and regret bound.	Moreover, $\mathcal{A}'$ does not play any null-action before stopping.
%	\end{remark}
%	
%	\begin{remark}
%		\label{rem:UCBNullArm}
%		To obtain the stated regret bounds in Theorem~\ref{thm:logRegretUpper} we first upper-bound the number of time-steps in which the algorithm chooses an action $a$ from distribution $\vec{X}_t$ such that $\supp(\vec{X}_t) \neq \supp(\vec{X}^*)$. Thus, in the remaining time-steps the algorithm chooses distributions $\vec{X}_t$ such that $\supp(\vec{X}_t) = \MainSet$. Using the strategy described in remark~\ref{rem:nullArm} we can ensure that $X_t(a^*) = 1 \geq X^*(a^*)$.
%	\end{remark}


==> checklist.tex <==
\section{Checklist}

\begin{itemize}
\item[(1a)] Q: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    A: Yes, also see Section~\ref{sec:significance} for additional discussion.

\item[(1b)] Q: Have you read the ethics review guidelines and ensured that your paper conforms to them?
A: Yes

\item[(1c)] Q: Did you discuss any potential negative societal impacts of your work?

A: This is a theoretical paper which elucidates regret bounds of an existing bandit algorithm, and advances theoretical understanding of multi-armed bandits. Thus, it is very unlikely to directly cause any negative societal impact. 

As this paper contributes to the field of bandit learning, it may indirectly contribute to whatever societal impact the entire field might have, both positive or otherwise. While we are not aware of any concrete evidence of actual or likely societal harms caused by bandit algorithms, it is important to be mindful that such harms might exist in some application scenarios. By definition, bandit learning trades off exploration vs exploitation, which in many applications means worsening the experience of some users for the sake of improving the aggregate experience of all users (\ie with positive societal effects). However, \citet{externalities-colt18} suggest artificial constructions in which users are served by a bandit algorithm, and the presence of one population of users creates a negative externality upon another.


\item[(1d)]  Q: Did you describe the limitations of your work?

A: Yes. Our theoretical results hold only for the model and assumptions as specified in the paper. Both the model and the assumptions are carefully spelled out (resp., in Introduction/Preliminaries and next to the respective theorems). Incidentally, the limitations of our positive results on logarithmic regret are in fact a ``feature", as we prove that such limitations are in fact inevitable for any algorithm.

\item[(2a)] Q: Did you state the full set of assumptions of all theoretical results?

A: yes, see above.
%A: Yes, the assumptions are encapsulated in Definition~\ref{def:best-arm-optimal} and Assumption~\ref{ass:LBAss} for the upper and lower-bounds respectively.

\item[(2b)]
Q: Did you include complete proofs of all theoretical results?

A: Yes. We provide full proofs for all results, either in the body of the paper or in the supplement. If the full proof is in the supplement, we include a proof sketch in the body.
	
\end{itemize}

Checklist items 3, 4, 5 not applicable to this paper.

==> logRegLowerBound.tex <==
%\vspace{-3mm}
\section{Lower Bounds [OBSOLETE!]}
\label{sec:lowerBoundLog}

We provide several lower bounds to complement Theorem~\ref{thm:logRegretUpper}. Essentially, we show that the $\Dmin^{-2}$ dependence is optimal, and that $d\leq 2$ resources and
best-arm-optimality are necessary. We present the theorems and intuition first; the proofs are exposed in the subsections.

\subsection{Results and intuition}

We consider problem instances with three arms $\{A_1,A_2,\nullArm\}$, Bernoulli rewards, and $d\geq 2$ resources, one of which is time; call them \emph{$3\times d$ instances}. Each lower bound constructs a pair of problem instances $\mI,\mI'$ such that any algorithm incurs high regret on at least one of them. The two instances are similar: they have the same parameters $T,K,d,B$, and the mean reward and the mean consumption for each arm and each resource differ by at most $\eps$; then, one instance is called an \emph{$\eps$-perturbation} of another. In fact, each lower bound exhibits a \emph{family} of such $\mI,\mI'$ pairs.

Our first lower bound concerns the dependence on $\Dmin$, and holds for any given value thereof.

\begin{theorem}[dependence on $\Dmin$]\label{thm:mainLB}
Posit an arbitrary time horizon $T$, budget $B = \nicefrac{T}{2}$, and $d=2$ resources (including time). For any
    $\eps\in(\nicefrac{1}{\sqrt{T}},\nicefrac{1}{4})$,
there exist two $3\times 2$ problem instances $\mI$, $\mI'$ with $\Dmin=\eps/2$ such that any algorithm incurs regret
$\OPTFD-\E[\REW] \geq \Omega\rbr{\Dmin^{-2}}$
on either $\mI$ or $\mI'$.
In fact, both problem instances have deterministic resource consumption.
\end{theorem}

The problem instances for Theorem~\ref{thm:mainLB} are constructed as follows. For arm $A_1$, resource consumption is deterministically  $\nicefrac{1}{2}$, and reward is drawn from
    $\term{Bernoulli}(\nicefrac{1}{4})$.
 For arm $A_2$, the consumption is deterministically $1$, and the reward is drawn from
    $\term{Bernoulli}(\nicefrac{1}{2} \pm \nicefrac{\eps}{2})$.
\footnote{That is, the reward for arm $A_2$ is
    $\term{Bernoulli}(\nicefrac{1}{2} + \nicefrac{\eps}{2})$
for one instance, and
    $\term{Bernoulli}(\nicefrac{1}{2} - \nicefrac{\eps}{2})$
for another.}
That $\Dmin$ is as claimed follows immediately from the construction.
Because of the small difference between the two instances, any algorithm will choose a ``wrong" arm at least $\Omega(\eps^{-2})$ times on one of the instances, which in turn implies $\Omega(\eps^{-2})$ regret. The full proof is in Section~\ref{sec:LB-gap}.

%	\begin{definition}		\label{def:epsPerturbed}
%An \emph{$\eps$-perturbation} of a BwK instance $\mI$ is a problem instance $\mI'$ which coincides with $\mI$ except in the reward distribution of one arm, so that its expected reward is changed by at most $\eps$.
%	\end{definition}

\vspace{2mm}

Next, we argue that regret $\Omega(\sqrt{T})$ is essentially inevitable if a problem instance $\mI_0$ is far from best-arm-optimal \asedit{or if there are $d>2$ resources. For both results, we construct two problem instances $\mI,\mI'$ that are small perturbations of $\mI_0$, and prove that any algorithm suffers high regret on one of them.} This is a fairly general result: unlike many bandit lower bounds that focus on a specific problem instance, we allow a wide range of instances $\mI_0$, as per the following assumption.


% in a substantial way, in in the sense that an optimal distribution puts at least a constant probability on (at least) one of the non-null arms.

\newcommand{\cLB}{c_{\mathtt{LB}}}

\begin{assumption}\label{ass:LBAss}
There exists an absolute constant $\cLB\in (0,\nicefrac12)$ such that:
\begin{enumerate}

\item \label{boundReward} $r(A_i),\,c_j(A_i)\in (\cLB,\,1-\cLB)$
for each arm $i\in \{1,2\}$ and each resource $j$.

\item \label{rewardDiff} $r(A_2) - r(A_1) \geq \cLB$ and $c_j(A_2) - c_j(A_1) \geq \cLB$ for every resource $j \in [d]$.
		
\item \label{nonNegativity} Mean consumption is strictly positive:
$c_j(A_i) > 0$ for each arm $A_i$ and resource $j \in [d]$.

\item \label{boundOPT} $\OPT - B \geq \cLB\cdot T$.

\item \label{boundLagrange} Lagrangian gap is not extremely small:
$\Dmin \geq \cLB/\sqrt{T}$.

\end{enumerate}
\end{assumption}


\begin{theorem}\label{thm:LB-root}
Posit an arbitrary time horizon $T$, budget $B$, and $d$ resources (including time). Fix any $3\times d$  problem instance $\mI_0$ which satisfies Assumption~\ref{ass:LBAss}. Assume either one of the following:
\begin{OneLiners}
\item[(a)] \label{cor:bestArmOptimal}
$d=2$ and $\mI_0$ is far from being best-arm-optimal, in the sense that
\begin{align}\label{eq:cor:bestArmOptimal}
\text{There exists an optimal solution $\vec{X}^*$ such that
$X(A_1)>0$ and $X(A_2) \geq \cLB$.}
\end{align}


\item[(b)] \label{cor:multipleResources} $d>2$

\end{OneLiners}

\noindent Then there exist problem instances $\mI,\mI'$, which are
$\mathcal{O}\rbr{\nicefrac{1}{\sqrt{T}}}$-perturbations of $\mI_0$, such that
\begin{align}\label{eq:LB-guarantee}
\text{Any algorithm incurs regret
    $\OPTFD-\E[\REW] \geq \Omega\rbr{ \cLB^{-4}\; \sqrt{T}}$
on $\mI$ or $\mI'$}
\end{align}
\end{theorem}


%\begin{theorem}[Best-arm-optimality is necessary]
%\label{cor:bestArmOptimal}
%Posit an arbitrary time horizon $T$, budget $B$, and $d=2$ resources. Fix any $3\times 2$  problem instance \asedit{$\mI_0$} which satisfies Assumption~\ref{ass:LBAss} with constant $\cLB$. Suppose that \asedit{$\mI_0$} is sufficiently far from being best-arm-optimal, in the following sense:
%\begin{align}\label{eq:cor:bestArmOptimal}
%\text{There exists an optimal solution $\vec{X}^*$ such that
%$X(A_1)>0$ and $X(A_2) \geq \cLB$.}
%\end{align}
%
%\noindent Then there exist $3\times 2$ problem instances $\mI,\mI'$, where $\mI$ is a mean-twin of $\mI_0$ and $\mI'$ is an $\mathcal{O}\rbr{\nicefrac{1}{\sqrt{T}}}$-perturbation
%thereof, which satisfy \eqref{eq:LB-guarantee}.
%%   $\eps \in \sbr{0, \mathcal{O}\rbr{ 1/\sqrt{T} }}$,
%%such that any algorithm incurs regret
%%    $\OPTFD-\E[\REW] \geq \Omega\rbr{ \cLB^{-4}\; \sqrt{T}}$
%%on one of these instances.
%\end{theorem}
%
%Finally, we argue that $\Omega(\sqrt{T})$ regret is inevitable with $d>2$ resources. This is a general result: we start with an arbitrary $3\times d$ problem instance $\mI_0$ under the mild restrictions of Assumption~\ref{ass:LBAss}. We prove that any algorithm incurs large  regret on a small perturbation of $\mI_0$: we construct two small perturbations of $\mI_0$, and each algorithm incurs large regret on at least one of them.
%
%\begin{theorem}[$d=2$ is necessary]
%\label{cor:multipleResources}
%Posit an arbitrary time horizon $T$, budget $B$, and $d>2$ resources (including time). Fix any $3\times d$ problem instance $\mI_0$ which satisfies Assumption~\ref{ass:LBAss} with constant $\cLB$. Then there exist problem instances $\mI,\mI'$, which are
%$\mathcal{O}\rbr{\nicefrac{1}{\sqrt{T}}}$-perturbations of $\mI_0$, such that any algorithm incurs regret $\OPTFD-\E[\REW] \geq \Omega( \sqrt{T})$ on ether $\mI$ or $\mI'$.
%	\end{theorem}

\begin{remark}
The problem instances in the theorem require randomized resource consumption. This is crucial for part (b) given our positive result for deterministic consumption (Theorem~\ref{thm:deterministic}). \asedit{For part (a), instance $\mI$ has the same expected outcomes as $\mI_0$ (but possibly different outcome distributions); we call such problem instances \emph{mean-twins}.}
\end{remark}
	
Both parts of Theorem~\ref{thm:LB-root} are corollaries of a more generic lower bound for $3\times d$ problem instances which focuses on linear independence of per-resource consumption vectors
\begin{align}\label{eq:per-resource-vector}
 \vec{c}_j  := \rbr{ c_j(A_1),\, c_j(A_2),\, c_j(\nullArm)} \in [0, 1]^3,
 \quad \text{resources $j\in[d]$}.
 \end{align}
	\begin{theorem}\label{thm:generalLB}
		Posit an arbitrary time horizon $T$, budget $B$, and $d\geq 2$ resources (including time). Fix any $3\times d$ problem instance $\mI_0$ that satisfies Assumption~\ref{ass:LBAss} and \refeq{eq:cor:bestArmOptimal}. Assume that the consumption vectors in \refeq{eq:per-resource-vector} are linearly independent. \asedit{Then there are instances $\mI,\mI'$ which are $\eps$-perturbations of $\mI$, with
    $\eps = \rbr{ \nicefrac{\cLB^2}{(1-\cLB)} } / \sqrt{T}$,
which satisfy \eqref{eq:LB-guarantee}. In fact, $\mI$ is a mean-twin of $\mI_0$.}
%such that any algorithm incurs regret
%$\OPTFD-\E[\REW] \geq \asedit{\Omega\rbr{ \cLB^{-4} \cdot \sqrt{T}}}$
%on $\mI$ or $\mI'$.
%on one of the two problem instances.
	\end{theorem}

\newcommand{\NewI}{\widetilde{\mI}_0}

The corollaries are obtained as follows. For Theorem~\ref{thm:LB-root}(a), problem instance $\mI_0$ trivially satisfies all preconditions in Theorem~\ref{thm:generalLB}.
Indeed, letting time be resource $1$, the per-resource vectors are
    $\vec{c}_1 = (0,0,1)$
and
    $\vec{c}_2 = (\,\cdot\,,\,\cdot\,,\,0)$,
hence they are linearly independent. For Theorem~\ref{thm:LB-root}(b), we use some tricks from the literature to transform the original problem instance $\mI_0$ to another instance $\NewI$ which satisfies
\refeq{eq:cor:bestArmOptimal} and the linear independence condition.
The full proof is in Section~\ref{sec:LB-d}.

The intuition for Theorem~\ref{thm:generalLB} is as follows. Given an instance $\mI_0$, the instance $\mI'$ is constructed as follows: for arm $A_2$, mean consumption on all resources except time is increased by
    $\mathcal{O}\rbr{\nicefrac{1}{\sqrt{T}}}$,
and everything else stays the same. \ascomment{TODO: insert one sentence to explain $\mI$.}
Because of the small difference between the two instances, any algorithm will choose a sufficiently ``wrong" distribution over arms sufficiently often. The assumption in \refeq{eq:cor:bestArmOptimal} and the linear independence condition are needed to ensure that ``wrong" algorithm's choices result in large regret. The full proof is in Section~\ref{sec:LB-generic}.



\OMIT{ %%%%%%%%%
\kaedit{The problem instances for Theorem~\ref{cor:multipleResources} is constructed as follows. Define
	\[	\zeta_1 := \min \left \{ \tfrac{1}{\sqrt{T}}, \{c_j(A_i)\}_{j \in [d], i \in [2]}, \frac{1}{(d!)^2} \right \}, \qquad and
	\]
	\[
		\zeta_2 := \min \left\{ \{c_j(A_i)\}_{j \in [d], i \in [2]}, \tfrac{1}{\sqrt{T}} \right \}.
	\]
	Given instance $\mI_0$, we construct instance $\mI$ by decreasing the mean consumption on arm $A_i$ and resource $j$ (except time) by $\zeta_1^j + u_j(A_i)$ where $u_j(a) \sim [-\zeta_2, \zeta_2]$ uniformly at random. We keep the mean rewards the same. As before $\mI'$ is obtained from $\mI$ by decreasing the mean consumption on all resources, except time, of one arm (say $A_2$) by $\eps = \mathcal{O}\left(\frac{1}{\sqrt{T}}\right)$ while keeping all other mean rewards/consumptions the same as in $\mI$.}
} %%%%%%%



%\kaedit{The problem instances for Theorem~\ref{thm:generalLB} is constructed similar to that for Theorem~\ref{cor:bestArmOptimal}.}



%
%\begin{theorem}	\label{thm:lowerBound}
%Fix an arbitrary time horizon $T$ and budget $B\geq \Omega(T)$. Fix any $3\times 2$ problem instance such that (i) $r(A_2) - r(A_1) \geq \Omega(1)$, $c_1(A_2) - c_1(A_1) \geq \Omega(1)$ (ii) $\OPT \geq 2B$, and (iii) some optimal solution $\vX^*$ to LP~\eqref{lp:primalAbstract} puts at least a constant probability on each non-null arm. Let $\mI'$ be an $\eps$-perturbation of $\mI$, where $\eps$ is an absolute constant times $\tfrac{1}{\sqrt{T}}$. Then any algorithm incurs regret
%$\OPTFD-\E[\REW] \geq \Omega( \sqrt{T})$.
%	\end{theorem}
%	


==> other-conf.tex <==
\section{Simple regret of \UCBBwK algorithm [OBSOLETE!!!]}

\asedit{We define \emph{simple regret} in a given round $t$ as
    $\OPTDP/T- r(\vX_t)$,
where $\vX_t$ is the distribution over arms chosen by the algorithm. The benchmark $\OPTDP/T$ generalizes the best-arm benchmark from stochastic bandits. If each round corresponds to a user and the reward is this user's utility, then $\OPTDP/T$ is the ``fair share" of the total reward. We prove that with \UCBBwK, all but a few users receive close to their fair share. This holds if $B>\Omega(T) \gg K$, without any other assumptions.}

\begin{theorem}\label{thm:UCBSmallNonArms}
Consider \UCBBwK. Assume $B \geq \Omega(T)$ and $\myEta\leq \tfrac12$. With probability $\geq 1-O(T^{-3})$, for each $\eps>0$, there are at most
$N_\eps = \mathcal{O}\left( \frac{K}{\eps^2} \log KTd  \right)$ rounds $t$ such that
    $\OPTDP/T - r(\vX_t) \geq \eps$.
\end{theorem}

%We provide a new analysis of \UCBBwK, building on another, technically different generalization of reward-gap. This generalization, called \emph{LP-gap}, applies to distributions over arms (rather than individual arms), and measures the difference in LP-value compared to the optimal distribution. One crucial argument concerns the ``confidence sums": the sums of confidence terms of the arms (or distributions over arms) chosen by the algorithm.


To prove Theorem~\ref{thm:UCBSmallNonArms}, we consider another generalization of the ``reward-gap", which measures the difference in LP-value compared to $\OPTLP$. For distribution $\vX$ over arms, the \emph{LP-gap} of $\vX$ is
\begin{align}\label{eq:LPgap-defn}
\Gap(\vX) := \OPTLP - \Val(\vX), \;\text{where}\;
V(\vX) := \textstyle (\nicefrac{B}{T})\;\cdot r(\vX)  / \rbr{\max_{j\in [d]} c_j(\vX)}.
\end{align}
Here, $V(\vX)$ is the value of $\vX$ in the LP~\eqref{lp:primalAbstract} after rescaling.
%    $ V(\vX) := \nicefrac{B}{T}\;\cdot r(\vX)  / \max_{j\in [d]} c_j(\vX)$.
%The LP-gap of $\vX$ is defined as
%    $\Gap(\vX) := \OPTLP - \Val(\vX)$.
It suffices to study the LP-gap because
    $r(\vX_t)\geq \Val(\vX_t) (1-\myEta)$
for each round $t$ with high probability. This holds under the ``clean event" in \eqref{eq:cleanEvent}, because $\vX_t$ being the solution to the optimistic LP implies
    $\max_j c_j(\vX_t) \geq \nicefrac{B}{T}\; (1-\myEta)$.

Thus, we upper-bound the number of rounds $t$ in which $\Gap(\vX_t)$ is large. We do this in two steps, focusing on the confidence radius $\rad_t(\vX_t)$ as defined in \eqref{eq:MaxConfRadUB}. First, we upper-bound the number of rounds $t$ with large $\rad_t(\vX_t)$. \asedit{A crucial argument concerns \emph{confidence sums}:
\begin{align}\label{eq:confSums}
\textstyle
\sum_{t \in S}\; \rad_t(a_t)
\quad\text{and}\quad
\sum_{t \in S}\; \rad_t(\vX_t),
\end{align}
the sums of confidence radii over a given subset of rounds $S\subset [T]$, for, resp., actions $a_t$ and distributions $\vX_t$ chosen by the algorithm.} Second, we upper-bound $\Gap(\vX_t)$ in terms of $\rad_t(\vX_t)$. The details are spelled out in Appendix~\ref{app:simple-regret}.

\newpage
\section{Reduction from \BwK to stochastic bandits}

\asedit{We improve all regret bounds for \UCBBwK algorithm, from worst-case regret to logarithmic regret to simple regret, when the problem instance has some helpful structure. In fact, we provide a general \emph{reduction} which translates insights from stochastic bandits into results on \BwK. This reduction works as follows: if prior work on a particular scenario in stochastic bandits provides an improved upper bound on the confidence sums \eqref{eq:confSums},
this improvement propagates throughout the analyses of \UCBBwK.} Specifically, suppose
    $\sum_{t\in S} \rad_t(a_t) \leq \sqrt{\beta\, |S|}$
for all algorithms, all subsets of rounds $S\subset [T]$, and some instance-dependent parameter $\beta\ll K$,
then \UCBBwK satisfies
\begin{OneLiners}
\item[(i)] worst-case regret
  $\OPTDP -\E[\REW] \leq O(\sqrt{\beta T})(1+\OPTDP/B)$.

\item[(ii)]
Theorem~\ref{thm:logRegretUpper} holds with
    $\Psi = \beta\,\Dmin^{-2}$
and regret
    $\mO\rbr{ \beta\,\Dmin^{-1} }$
in part (ii).

\item[(iii)] Theorem~\ref{thm:UCBSmallNonArms} holds with
$N_\eps = \mO\left( \beta\,\eps^{-2}  \right)$.
\end{OneLiners}			
\asedit{Conceptually, this works because confidence sum arguments depend only on the confidence radii, rather than the algorithm that chooses arms, and are about stochastic bandits rather than \BwK. The analyses of \UCBBwK in \citep{AgrawalDevanur-ec14} and the previous sections use $\beta=K$, the number of arms. The confidence sum bound with $\beta=K$ and results (i, ii, iii) for stochastic bandits follow from the analysis in \cite{bandits-ucb1}.}

%The conceptual contribution here is to identify the right mathematical structure: the bound on the confidence sum; the technical details are easy.

We apply this reduction to three well-studied scenarios in stochastic bandits:
combinatorial semi-bandits
\citep[\eg][]{Chen-icml13,Kveton-aistats15,MatroidBandits-uai14},
linear contextual bandits
\citep[\eg][]{Auer-focs00,DaniHK-colt08,Langford-www10,Reyzin-aistats11-linear,Csaba-nips11},
and multinomial-logit (MNL) bandits \citep{Shipra-ec16}.
The confidence-sum bounds are implicit in prior work on stochastic bandits, and we immediately obtain the corresponding extensions for \BwK. To put this in perspective, each scenario has lead to a separate paper on  \BwK \citep[resp.,][]{Karthik-aistats18,agrawal2015linear,Cheung-MNLBwK-arxiv17}, for the worst-case regret bounds alone. We match the worst-case regret bounds from prior work, and obtain new bounds on logarithmic regret and simple regret. The details are spelled out in Appendix~\ref{sec:extensions}.

Another reduction from \BwK to bandits, found in \cite{AdvBwK-focs19}, is very different from ours. It requires a much stronger premise (a regret bound against an adaptive adversary), and only yields worst-case regret bounds. Moreover, it reuses a bandit algorithm as a subroutine, whereas ours reuses a lemma.
% whereas ours reuses a lemma about confidence sums.

